A Component-Based Formal Language Workbench

The CBS framework supports component-based specification of programming languages. It aims to significantly reduce the effort of formal language specification, and thereby encourage language developers to exploit formal semantics more widely. CBS provides an extensive library of reusable language specification components, facilitating co-evolution of languages and their specifications. After introducing CBS and its formal definition, this short paper reports work in progress on generating an IDE for CBS from the definition. It also considers the possibility of supporting component-based language specification in other formal language workbenches.

==> eptcsdata.tex <==
\providecommand{\firstpage}{29}
\providecommand{\publicationstatus}{R. Monahan, V. Prevosto, J. Proen\c{c}a (Eds.): Formal\\
Integrated Development Environment 2019 (F-IDE 2019)\\
EPTCS 310, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.310.4}{10.4204/EPTCS.310.4}}
\pdfoutput=1

